Cross-Task Generalization via Natural Language Crowdsourcing Instructions

Humans (e.g., crowdworkers) have a remarkable ability in solving different tasks, by simply reading textual instructions that define them and looking at a few examples. Despite the success of the conventional supervised learning on individual datasets, such models often struggle with generalization across tasks (e.g., a question-answering system cannot solve classification tasks). A long-standing challenge in AI is to build a model that learns a new task by understanding the human-readable instructions that define it. To study this, we introduce NATURAL INSTRUCTIONS, a dataset of 61 distinct tasks, their human-authored instructions, and 193k task instances (input-output pairs). The instructions are obtained from crowdsourcing instructions used to create existing NLP datasets and mapped to a unified schema. Using this meta-dataset, we measure cross-task generalization by training models on seen tasks and measuring generalization to the remaining unseen ones. We adopt generative pre-trained language models to encode task-specific instructions along with input and generate task output. Our results indicate that models benefit from instructions when evaluated in terms of generalization to unseen tasks (19% better for models utilizing instructions). These models, however, are far behind an estimated performance upperbound indicating significant room for more progress in this direction.

==> comments-copied-here.tex <==
% old intro: 

\citet{mccarthy1960programs} in his seminal work outlined a hypothetical machine that accepts \emph{instructions} in the form of  declarative knowledge as  input and incorporates them in its decision-making. It is hard to achieve this vision with the dominant supervised learning paradigm that uses task-specific labeled data to train models which usually cannot generalize to new tasks. Most recently,  large pre-trained language models \cite{brown2020language} show successful results when they are provided with a natural language prompt and a few task-specific  examples. However, these  tasks and required language prompts  are often  simpler than comprehensive instructions required for complex NLP tasks (e.g.,  \hanna{cite some of the datasets we used in our paper that gpt3 cannot perform well}). In fact, a recent study~\cite{efrat2020turking} show that these  models fail to learn three complex tasks (SQuAD, .... \hanna{give those examples}) given their crowdsourcing instructions.  %\cite{raffel2020exploring,brown2020language}
\begin{figure}[t]
    \centering
    % \includegraphics[scale=0.87, trim=0.5cm 0.7cm 0cm 0.5cm]{figures/intro-teaser.pdf}
    \includegraphics[scale=0.81, trim=0.5cm 0.7cm 0cm 0.5cm]{figures/intro-teaser-2.pdf}
    \caption{
        \name{} contains a variety of tasks, each accompanied by their natural language instructions. A model is expected to \emph{understand} the given {\color{blue} instructions} and answer {\color{darkgreen} the given input} accordingly. 
        Models that make appropriate use of the instructions can generalize to \emph{unseen} tasks. 
        % \hanna{figure improvement: the robot box in the middle should be much smaller and a bit wider; you are losing too much white space here; need to highlight instruction; also what is an input? that's an input to the task, but the input to our model is the full box of instruction+input. Be careful and cocrete about these tems.} 
    }
    \label{fig:teaster}
\end{figure}

Humans are often capable of following these instructions, leading to many large-scale datasets created through crowdsourcing. Figure~\ref{fig:teaster} shows some example instructions that  describe three NLP tasks for a given paragraph, varying from  \emph{classifying} a paragraph to,
\emph{modifying an input sentence}, \emph{answering} questions.  


In this paper, we study if models equipped with understanding natural language instructions can be generalized to new tasks,  revisiting McCarthy's vision of enabling machines to perform tasks given instructions. 
We build a dataset consisting of crowdsourcing instructions for tasks and their instances, where instructions are represented with an underlying schema. We use our dataset to build and systematically evaluate models that can learn tasks from instructions with no task-specific labeled data. % and systematically evaluate if  models equipped with understanding natural language instructions can  be generalized to new tasks. 

We introduce \name{}, a high-quality dataset of 61 distinct NLP tasks, each comprised of comprehensive instructions and several task instances. Inspired by~\citet{efrat2020turking}, we leverage
crowdsourcing instructions of existing NLP datasets to construct \name{}. In contrast to \citet{efrat2020turking},
\name{} includes a  diverse set of tasks whose instructions are all mapped to a unified schema,  which enables building models  that generalize across different tasks. Moreover, tasks  in \name{} are defined as minimal stand-alone steps in the crowdsourcing instructions provided to humans. For example, the tasks in Quoref~\cite{dasigi2019quoref} is split into two tasks of question generation and answer generation, mimicking its data collection process by humans.

We build models  trained to follow instructions for tasks in \name{} training and evaluate if they can generalize to follow instructions for  new tasks under different settings.  Our models use generative language models BART~\cite{lewis2019bart} and GPT-3~\cite{brown2020language}, encode the input instruction into textual formats and decode an output text.  Our evaluation of 
these models indicates that natural language instructions 
improve the generalization to unseen
tasks, even thought they have not used any task-specific annotated data. 

This pleasant surprise
stands in contrast to the findings of \citet{efrat2020turking} who did not observe any benefit in using instructions.   We hypothesize that the shown benefits here are due to our formulation (minimal instructions mapped into schemas) and the scale of tasks included in \name. 
\daniel{TO BE UPDATED:}
Our models generally benefit from instructions, however, we find that these gains are sensitive to various parameters, such as the semantics of the task at hand (Fig.\ref{fig:gains:per:categories}).  
Ablations (\S\ref{sec:ablation:study}) indicate that GPT-3 gains notably from positive examples, mildly benefits from the task definitions, and tends to be confused about negative examples or `things to avoid' instructions. 
\begin{comment}
Similarly, models are sensitive to how the instructions are phrased. 
Using this intuition, we present general procedures to \emph{calibrate} the instructions for each task, which lead to improvements in their performance. \daniel{is this clear?}
\end{comment}

Despite the benefits of instructions, 
we find that there is a sizable gap between models' performance and
their oracle upper-bound estimates,
indicating a substantial room to progress. 
We hope this gap, as well as the availability of \name{} will encourage development of stronger models of language. 





\textbf{Contributions:} In summary, the contributions of this work are as follows: 
(a) we introduce \name{}, a large dataset of human-authored
instructions  curated from existing well-known datasets mapped to unified schema; 
(b) we benchmark state-of-the-art models and show better cross-task generalization by leveraging instructions; 
(c) we conduct a variety of analyses which show the sensitivity of the models to the target task and the elements of the instruction. 





\chitta{Should we say something like: ``Besides imperative natural language statements about what to do, instructions also include additional information such as a small set of examples.'' This can be said in the caption of Fig 1. We may cite https://www.jstor.org/stable/30220664?seq=1 . This becomes clear later in the paper in Section 3; but did confuse me when I first came across it. Also, McCarthy's notion of instructions in his 1960 paper did not have these additional aspects. So another citation about what an ``instruction'' is, may be helpful.} 


\begin{comment}
The instruction paradigm~\cite{goldwasser2014learning,efrat2020turking} is a strict generalization of the current ``no-instructions'' paradigm. 
With the saturation of the existing benchmarks~\cite{wang2019superglue} that follow the conventional paradigm, we believe the field should move towards models that can address a \emph{broader} range of tasks.
Learning to follow \emph{instructions} is one alternative that brings in more generality to our models and it remains to be challenging to our models. 
\end{comment}

%However, models equipped with understanding and reasoning with \emph{natural language instructions}~\cite{goldwasser2014learning,weller-etal-2020-learning} should be able to generalize to any task that can be defined via instructions. 
% Towards this goal, we build upon the work of~\citet{efrat2020turking} who use crowdsourcing instructions as a challenge for NLP models, however observed very minimal benefit from instructions. 
% One central hurdle towards towards studying this goal is the lack of large-scale benchmarks with natural and high-quality instructions, as the existing ones are either unrealistically simple~\cite{weller2020learning} or too small~\cite{efrat2020turking}. 


%\swaroop{Recently, \cite{weller2020learning} proposed the ZEST dataset to learn from task descriptions. However, their description is limited to common questions someone might ask about three different domains: U.S. presidents, dog breeds, and U.S. national parks. On the other hand, \cite{efrat2020turking} proposed the Turking Test where they asked models to follow natural language instructions. However, the Turking Test expects models to address all crowdsourcing instructions at once which is a very difficult task to follow \cite{efrat2020turking}. Also, the scope of their study was limited as they only studied 3 datasets. We aim to address these three issues by building a diverse dataset that covers natural instructions beyond questions. We divide each task into various subtasks so that it becomes relatively easier for models to follow. Finally we conduct our study with large-scale data to appropriately evaluate model's response to instructions.}

\begin{comment}
\newcommand{\setup}[1]{$\mathcal{S}_{#1}$}

\begin{table}[h]
    \centering
    \small
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{cl}
        \toprule
        Setup & Description \\
        \midrule
        % \cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-3} 
        \setup{1} & random split of tasks   \\ 
        \setup{2} & leave-one-category generalization \\ 
        \setup{3} & leave-one-dataset-out generalization \\ 
        \setup{4} & leave-one-task-out generalization \\ 
        \bottomrule
    \end{tabular}
    % }
    \caption{
        Different splits considered in this work. Each split measures a slightly different form of generalization.          % Different modes of supervision considered in this work, when evaluating a model on the instances of a fixed task $T \in$ \task{eval}. \daniel{needs to be updated. }
    }
    \label{tab:supervision:types}
\end{table}
\end{comment}


\begin{comment}
\paragraph{Step-wise vs shared instructions.}
In the case of QASC, the instruction size associated with each step of the data creation process is very high, whereas for Winogrande, it is exactly the opposite-- instruction size associated with each step of data creation process is very low. Instead, the size of the common instruction (i.e., the instruction preceding the first step of the data creation process) is high in Winogrande; this is  also seen for DROP. The major mode of instruction varies across datasets. 
Examples and instructions associated with each step of data creation respectively take up the majority of space in Quoref and CosmosQA.  
MCTACO relies on examples to explain the crowdsourcing task, while Winogrande and QASC depend mostly on common instructions and instructions associated with each step of the data creation process respectively, to explain the task to the crowdworker.
\daniel{not sure how to say this}
\end{comment}


\begin{comment}
\begin{itemize}
    \item \textbf{Representing a task \daniel{`a task'?} with all possible examples exhaustively is practically infeasible for a real NLP task. Instructions on the other hand represents the broad view of the task and underlying concept which sort of get diluted or biased when grounded with examples.
    } E.g We want to teach concepts such as temporal reasoning associated with event duration. \daniel{should not be in your first paragraph:} We create detailed crowdsourcing instructions which helps crowdworkers understand the task and create data samples. Next, we throw away the instructions, feed dataset to models 90 \% of which starts with 'how long' \daniel{?}. So, machines just overfit to these examples instead of learning the actual task of temporal reasoning. \daniel{this is verbose paragraph. Can you summarize the argument in 1-2 sentence? It might help to cite the recent work to justify why it is important to focus on instructions.}
    \item \textbf{Instructions provide the flexibility to explicitly state facts} \daniel{here you can mention the classic works on `declarative learning' e.g., \cite{?} } e.g. negations which we only hope to express implicitly through examples.
    \begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/intro.png}
    \caption{Example vs Instruction Paradigm Illustration}
    \label{fig:Intro_diagram}
    \end{figure}
    \begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/comp.png}
    \caption{CEP vs IP Comparison \daniel{You can use this in your slides, but not in your academic papers} }
    \label{fig:Intro_diagram}
    \end{figure}
    \item \textbf{Instructions are user-friendly \daniel{human readable?}, so anyone can leverage NLP bringing machines closer to humans; right now NLP applications are limited to experts.} This expands the range of NLP applications which is inline with our progress superivised learning, transfer learning, fewshot learning--> learning from instructions. In fact, we often don't know the answer to the questions we need answer for e.g. some calculation, write a story, ask what's the best decision. Machine Learning with examples limits usage as we need to know the answer, so Instruction is important.
    \item \textbf{However, there exist no benchmark dataset to study model response to instructions. Also, there are no flexible schema to represent Instructions.} 
    \item \textbf{Building and Evaluating Natural Instructions:} We collect crowdsourcing instructions keeping in mind various skills required for designing a new task. We filter and curate these with the intention of building a toolbox of dataset creation tools. Raw instructions are unstructured, and lengthy (otften redundant) and also noisy that will not fit in to the token size of model. They are also multistep, so hard to follow. We decompose into multiple subtasks, came up with a schema to represent Instructions. Results on GPT-3 fewshot learning shows that Models are bad at responding to Instructions, it is indeed a challenge in the regions of extremely low sample complexity. We propose calibration and machines can do well with the right instruction. We incorporate human in the loop and show that the diversity etc. is as good as the original dataset with appropriate instructions. We promote this paradigm of feature engineering-architecture engineering-prompt engineering
    \item \textbf{Contributions:} (1) Schema, (2) Curated dataset (3) GPT-3 Fewshot, Finetuned BART(4) Calibration 
\end{itemize}
\end{comment}




%\paragraph{Instruction-augmented models.}
%In our setup, in addition to the instances $(X_t, Y_t)$, each task $t$ comes with instruction $I_t$. A given model $M$ is expected to map a given instruction $I_t$ and an input instance $X_t$ to its corresponding output $Y_t$: 

%\begin{equation}
%\label{eq:supervision}
%M: (I_t, X_t) \rightarrow Y_t.
%\end{equation}
 

\begin{comment}
\begin{equation*} 
    \begin{split}
        & \mathtt{for \; p \; in \;} \I{t}{pos. ex.}  \\ 
        & \hspace{0.5cm}  enc_2(I_t, x)  \pluseq \\ 
        & \hspace{0.99cm} \textnormal{``}\mathtt{\small Positive Example-}\mathtt{\small input:} \; \mathtt{p}_{\textnormal{\tiny input}}  \\ 
        & \hspace{0.99cm}  \; \mathtt{\small output:} \; \mathtt{p}_{\textnormal{\tiny output}} \; \mathtt{\small reason:} \; \mathtt{p}_{\textnormal{\tiny reason}} 
        \textnormal{''} 
    \end{split}
\end{equation*}
\end{comment}

\begin{comment}
\begin{table}[t]
    \centering
    % \includegraphics[scale=0.65,trim=1.7cm 7.9cm 0cm 2cm]{figures/results-table.pdf}
    % \includegraphics[scale=0.75,trim=3.4cm 14.0cm 0cm 2cm]{figures/results-table-1.pdf}
    \includegraphics[scale=0.65,trim=7.9cm 11.4cm 0cm 1.9cm]{figures/results-table-1.pdf}
    \caption{
        Empirical results \name{}. 
        % The best numbers among the four encodings are \underline{underlined}. 
        % The best number in each column is indicated with \textbf{bold}. 
        The first row is a task-specific model with no instances. This model serves as our upper-bound, which is why it is  {\color{gray} grayed out}.
        For each of the two systems (BART and GPT3), we see that the addition of the instructions helps propel the model performance, as indicated by the relative gains (the last column) compared to \greentext{their base encoding}.  
    }
    \label{tab:results:1}
\end{table}
\end{comment}

\begin{comment}
\begin{table*}[h]
    \centering
    \small
    \resizebox{2\columnwidth}{!}{
    \begin{tabular}{p{5cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.25cm}|p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.25cm}}
        \toprule
        model$\rightarrow$ &\multicolumn{7}{c}{BART}&\multicolumn{7}{c}{GPT-3}\\
        \midrule
        encoding$\downarrow$   task category$\rightarrow$ &QG&AG&CF&IAG&TM&VF&avg&QG&AG&CF&IAG&TM&VF&avg\\
        \midrule
        % \cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-3} 
      \textit{instance-only} & 26	&0.18&	6&	0.06&	0&	0.03&	21&	0.08&	33&	0.39&	7&	13&	0.08&	-&	-&	-&	-&	-&	-&	-&	-\\ 
        \textit{prompt}& 27&		22&		7&		22&		34&		9&	20&		33&		32&	14&	13&	73&	16&	30&\\
        \textit{prompt+definition} 35&	 24&	50&	25&	36&	7&	30&	36&	35&	40&	14&	70&	16&	35&\\
        \textit{prompt+things to avoid}& 33&		24&		4&		24&		58&		9&	25&		28&		33&	11&	16&	68&	14&	28&\\
        \textit{prompt+emphasis}& 38&		23&		16&		26&		49&		3&	26&		29&		28&	18&	16&	72&	16&	30&\\
        \textit{prompt+positive examples}& 56&		22&		28&	24&		53&		5&	31&		43&		49&	29&	21&	70&	36&	41&\\
        \textit{prompt+positive \& negative examples}& 50&		21&		27&		25&		50&		7&	30&		32&		19&	8&	12&	61&	13&	24&\\
        \textit{prompt+definition+ positive examples}& 55&		23&		50&		26&		54&		7&	36&		43&		50&	45&	23&	70&	32&	44&\\
        \textit{all instructions /\ examples}& 40&		24&		36&		25&		55&		8&	31&		31&		34&	39&	14&	69&	13&	33&\\
        \textit{positive examples}& 57&		6&		9&		25&		49&		7&	26&		30&		32&	15&	16&	68&	23&	31&\\
        \textit{all instructions /\ negative examples}& 53&	27&	53&	25&	48&	6&	35&	43&	54&	44&	21&	70&	32&	44&\\
        \textit{all instructions}& 46&	0.31&	25	0.13	52	0.14	25	0.11	35	0.6	7	32	0.11	33	0.23	18	8	12	60	11	24\\
    %   \textit{prompt} & 20&54\%&30& -  \\
    %   \textit{prompt+definition} &30&131\%&35&17\%\\
    %   \textit{prompt+things to avoid} &&&&\\

       
        % \setup{2} & leave-one-category generalization \\ 
        % \setup{3} & leave-one-dataset-out generalization \\ 
        % \setup{4} & leave-one-task-out generalization \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{
        Different splits considered in this work. Each split measures a slightly different form of generalization. 
        % Different modes of supervision considered in this work, when evaluating a model on the instances of a fixed task $T \in$ \task{eval}. \daniel{needs to be updated. }
    }
    % \label{tab:supervision:types}
\end{table*}
\end{comment}

% \begin{table}[h]
%     \centering
%     \small
%     % \resizebox{\columnwidth}{!}{
%     \begin{tabular}{lcccc}
%         \toprule
%         model$\rightarrow$ &\multicolumn{2}{c}{BART}&\multicolumn{2}{c}{GPT-3}\\
%         \midrule
%         Rouge-L$\rightarrow$ & avg&rel&avg&rel\\
        
%         encoding$\downarrow$&score&gains&score&gains\\
%         \midrule
%         % \cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-3} 
%       \textit{instance-only} & 13&-&-& -  \\ 
%       \textit{prompt} & 20&54\%&30& -  \\
%       \textit{prompt+definition} &30&131\%&35&17\%\\
%       \textit{prompt+things to avoid} &&&&\\

       
%         % \setup{2} & leave-one-category generalization \\ 
%         % \setup{3} & leave-one-dataset-out generalization \\ 
%         % \setup{4} & leave-one-task-out generalization \\ 
%         \bottomrule
%     \end{tabular}
%     % }
%     \caption{
%         Different splits considered in this work. Each split measures a slightly different form of generalization. 
%         % Different modes of supervision considered in this work, when evaluating a model on the instances of a fixed task $T \in$ \task{eval}. \daniel{needs to be updated. }
%     }
%     % \label{tab:supervision:types}
% \end{table}

 

%\paragraph{Data split within tasks.} For each task, we randomly create  training/dev/test splits (sized $6.5k/0.5k/1k$) and use the appropriate splits for supervision and evaluation. 
%The training sets are limited to $6.5k$ so that we don't have any issues related to data imbalance in our experiments. For tasks with less than $6.5k$ instances, we oversample via repetition.




% \subsection{Evaluating Generalization Across Tasks} 



\begin{comment}
\paragraph{\name{} tasks splits.}
To evaluate generalization across subtasks, we divide \name{} into two collections: 
(i) \emph{evaluation} tasks \task{eval}  (35 subtasks) for test and 
(ii) \emph{non-evaluation} tasks \task{non-eval}  (26 subtasks) for training.\footnote{The tasks are enumerated in the appendix.} 
% \hanna{this sentence is not clear-- revise}\daniel{better?}
In making this collection, we ensure that the tasks included in \task{eval} accept a relatively reliable automatic evaluation.  For example,  those tasks that have restricted answer space (like classification tasks) or those that have several gold output references. The end tasks of the source datasets which are typically the answer generation tasks are often included in the evaluation set.
% In making this collection, we ensure that the \emph{evaluation} subtasks accept a relatively reliable automatic evaluation (i.e., by having many gold output annotations for each input or having a limited space of output generations).
Additionally, we ensure to have at least one representative subtask from each of the semantic categories (\S\ref{sec:mapping}) in the \emph{non-evaluation} collection
% \st {so that the distribution of \emph{eval} and \emph{non-eval} subtasks are not vastly different from each other. } \swaroop{
However, tasks within categories are very different from each other. For instance, creation of DROP questions requires understanding of numerical reasoning and reading comprehension, whereas creation of Winogrande questions requires understanding of co-reference resolution and the requirement of the task to create twin question and answer pairs.

\daniel{
    emphasize that not any two tasks are exactly the same. Every two QG tasks are different (e.g., MC-TACO vs CosmosQA). 
}
\paragraph{Evaluation.}
We formulate three evaluation settings with different  supervision types available to a model (Table~\ref{tab:supervision:types}). 
In `task-specific' setting, a model is supervised with the training instances of the evaluation task -- similar to the conventional setup. 
In `few-shot' setting, a model  only observes a  few examples of the evaluation task.\footnote{
    We use ``few-shot'' to refer to \emph{any setup with a small number of labeled examples},
    % (the support set), 
    regardless of whether these examples are used for fine-tuning or inference-time conditioning (no gradient updates). 
}
In  `generalization' setting, a model does not observe any instances from the evaluation task.
\end{comment}



\begin{comment}
\paragraph {``no-instructions''} encoding.
This encoding is the conventional paradigm where no instructions exist, except the input instance (Eq.~\ref{}). 

\paragraph{\emph{``prompt''} encoding.}
In this encoding, we append the prompt message before the input instance. 

\paragraph{\emph{``prompt + definition''} encoding.}
In this encoding, the prompt message and the task \emph{definition} appear before the input instance.
Intuitively, this encoding is more informative and more complex than \emph{``prompt''} only encoding. 

\paragraph{\emph{``all instructions''} encoding.}
This encoding contains all the instruction content.
% \daniel{pos/negative don't have to have the same size.}
We include as many examples as possible, before exceeding the token limit of LMs. 

\paragraph{\emph{``positive examples''} encoding.}
This encoding contains only positive examples from the task instructions. 
% (no task description, etc.).  We fit as many positive examples as it fits in the input. 
Such example-only encodings have been used in several recent studies in prompting LMs~\cite{zhao2021calibrate}. 


\end{comment}

\begin{comment}
\begin{table}[h]
    \centering
    \small
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{L{1.9cm}cL{3.9cm}}
        \toprule
        Setup & Evaluation & Supervision \\
        \midrule
        % \cmidrule(r){1-1} \cmidrule(r){2-2} \cmidrule(r){3-3} 
        task-specific & $T \in$ \task{eval} & all the instances of $T$ \\ 
        \cmidrule(r){1-3} 
        few-shot & $T \in$ \task{eval} & 
        % \sout{few instances of $T$} \daniel{
        instructions of $T$ \\ 
        \cmidrule(r){1-3} 
        generalization & $T \in$ \task{eval} & instructions+ instances of \task{non-eval} tasks + instructions of $T$ \\ 
        % \cmidrule(r){1-3} 
        % weak generalization & $T \in$ \task{eval} & \task{non-eval} $\cup$  few instances of $T$ \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{
        Different modes of supervision considered in this work, when evaluating a model on the instances of a fixed task $T \in$ \task{eval}. 
    }
    \label{tab:supervision:types}
\end{table}
\end{comment}

\begin{comment}
\section{Evaluating Language Models to Address \name{}} 
% \hanna{re-orged and edited this section; make sure the section references are correct}

We use generative language models BART~\cite{lewis2019bart} and GPT-3~\cite{brown2020language} to address tasks in \name{}. Here, we describe how we encode instructions and instances into plain text and feed them into generative language models (\S \ref{subsect:encoding}). We then describe the model details (\S \ref{subsec:models}). 
We then explain how we use language models to encode instruction (\S \ref{subsect:encoding}). \daniel{to be updated}
\end{comment}

\begin{comment}
\paragraph{The benefit from instructions heavily depends on the task at hand.}
Figure~\ref{fig:gains:per:categories} shows the performance of our models on our task categories, broken down into several coarse input encodings. 
Similar to our previous observations, \emph{all instructions} encoding \emph{typically} performs better than other encodings. 
However, these gains are not uniform across task categories. 

% \paragraph{Instructions play a minimal role when the models are supervised with task-specific data.}


% \paragraph{Which Tasks Get Benefited the Most with Instructions?}
% \paragraph{How does fewshot learning with gradient update perform?}
% \paragraph{Which Tasks Get Benefited the Most with Instructions?}
% \paragraph{Which Tasks Get Benefited the Most with Supervised Learning?}
% Is there a correlation between Instruction Quality/details and the benefits
\end{comment}

\begin{comment}
\paragraph{Task-specific BART (oracle upper-bound estimate).}
% \swaroop{Can we remove the term upper-bound? I feel this is not really the upper-bound and can be crossed.}
We train BART on input/output instances of each task (no instructions) and evaluate on the same task. 
This is the conventional setup where the model is fine-tuned to solve the task only, without any instructions involved.
Such a model, by design, won't generalize across different tasks since it is specialized to each subtask. 
However, the numbers elicited from this can be viewed as the upper-bounds for each task (i.e., how well can BART perform, if it were to be trained on many instances of this particular task). 
%This model is listed in the first row of Table~\ref{tab:results:1}. 

% While out goal is to show generalization across subtasks, 
% The first baseline is BART trained on instances of each 
% We also calculate the oracle baseline using BART by relaxing the restriction of unseen tasks and allowing models to get trained on the large set of training instances. 
% We limit the usage of number of instance per subtask to 5k to evaluate model performance within a fixed computational budget which is a more realistic setup.
\end{comment}

\begin{comment}
\subsection{Task-specific Calibration of GPT-3}
\label{subsec:calibration}

We transform inputs (Instructions) to make it more understandable for GPT-3. We have a human-in-the loop setup to perform calibration. We do calibration in two steps (i) we develop various calibration procedure by experimenting with various type of prompts and identifying the types of prompt which help model follow instructions better. This is done on the non-eval split. (ii) we employ one of the calibration procedures by looking at few samples of the end-task in the eval split.
\end{comment}

\begin{comment}
\paragraph{A Data Creation Toolbox:} 
\name{} covers various skills beyond question generation and answer generation, such as sentence paraphrasing, verification of whether a question is in a specified category, etc that are frequently used during NLP dataset creation. A successful model trained on \textit{Natural Instructions} will be a toolbox for dataset creation. Our intuition behind the focus on dataset creation is that any NLP task can be expressed as a step in the data creation 
\end{comment}


==> old_text.tex <==
    % Humans (e.g., crowdworkers) have a remarkable ability in solving different tasks, by simply reading textual instructions that define them and looking at a few examples. NLP models built with the conventional paradigm, however, often struggle with generalization across tasks (e.g., a question-answering system cannot solve  classification tasks). A long-standing challenge in AI is to build a model that is equipped with the understanding of human-readable instructions that define the tasks, and can generalize to new tasks. To study this, we introduce NATURAL INSTRUCTIONS,  a dataset of 61  distinct tasks, their human-authored instructions and 193$k$ task instances. The instructions are obtained from crowdsourcing instructions used to collect  existing NLP datasets and  mapped to a unified schema.  We adopt generative pre-trained language models to encode task-specific instructions along with input and generate task output. Our results indicate that models can benefit from instructions to generalize across tasks. These models, however, are far behind supervised task-specific models, indicating significant room for more progress in this direction.
    
    
    
    % instructions and task-specific input/output data. 
% This dataset consists of 
% \changed{instructions for 61 distinct tasks}
% 61 distinct 
% instructional prompts 
% language instructions 
% and about 600$k$ task instances, 
% and is used to evaluate \changed{\sout{existing}} state-of-the-art language-models (LMs) in addressing new tasks by few-shot prompting of GPT3 and fine-tuning BART. 
% we observe that they are sensitive to task at hand, 
% are sensitive  to how the instructions are phrased. 
% We show how \emph{calibrating} the instructions for each model could remarkably improves their responses to instructional prompts; 

% NATURAL INSTRUCTIONS: Benchmarking Generalization to New Tasks from Natural Language Instructions
% Swaroop Mishra, Daniel Khashabi, Chitta Baral, Hannaneh Hajishirzi
% Can we enable NLP models to appropriately respond to instructional prompts and consequently generalize to new tasks? To study this question, we leverage the existing NLP datasets and the instructions that were used to crowdsource them to create NATURAL INSTRUCTIONS, a dataset of instructions and task-specific input/output data. This dataset consists of 61 distinct language instructions and about 600k task instances, and is used to evaluate existing state-of-the-art language-models (LMs) in addressing new tasks by few-shot prompting of GPT3 and fine-tuning BART. Our analysis indicates that: (a) the existing models indeed benefit from instructions and hence, show improved generalization to new tasks; (b) while models like GPT3 generally benefit from instructions, the extent of their gains varies across different fields of instructions and also depends on the task being solved; (c) generalization to unseen tasks in NATURAL INSTRUCTIONS remains far from perfect for the state-of-the-art, indicating significant room for more progress in this direction.


%(a) 
% the existing models \emph{benefit from instructions} and hence, show improved generalization to new tasks; 
% Models' generalization across tasks \emph{improves} with instructions. 
%Instructions boost models' generalization across tasks.
% (b) While models generally benefit from instructions, the gains are not uniform across subsets of the instructions: while task \emph{definitions} and \emph{positive examples} are most helpful, models often fail to utilize more abstract segments of instructions (such as \emph{negative examples}). 
% the extent of their gains varies across different fields of instructions and also depends on the task being solved; 
%(b) Generalization  to \emph{novel} tasks in \name{} remains far from perfect for the state-of-the-art, indicating significant room for more progress in this direction.\footnote{
% https://github.com/allenai/natural-instructions
%Dataset is available at [anonymous-URL]
%}


% \hanna{here, we need a sentence saying how you made these semantic categories and assigned them here}%We have categorized them into 7 semantic categories:  (1) \emph{question generation}, (2) \emph{answer generation}, (3) \emph{incorrect answer generation}, (4) \emph{classification}, (5) \emph{minimal text modification}, (6) \emph{long text generation}, and (7) \emph{verification}. 



%QASC contains detailed steps to create questions, whereas CosmosQA has high-level enumeration of desirable question attributes. 
%As mentioned in our desiderata (\S\ref{sec:design:considerations}), we view such variability as a desirable attribute of our instructions. 


 %given a context paragraph and a set of inst in the former a question is being generated given a context paragraph and a instructions, and in the latter an answer is being generated given a context paragraph and : is divided into two tasks of  (1) \emph{question generation} (input: context paragraph and instructions, output: question), and (2) \emph{answer generation} (input: context paragraph, instructions and question, output: answer). 
% Similarly, MCTACO's annotation crowdsourcing involves generating multiple types of questions, each with their own separate instructions. Therefore, we divide the task into multiple subtasks each representing a distinct type of question generation task. 
% Our intuition behind this whole process is to make the subtask definitions more consistent across various subtasks and hence, increasing the chances of success for the models.

% \begin{table*}[t]
%     \small 
%     \centering
%     \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccccc|l||cccccc|l}
% \toprule
% & \multicolumn{7}{c}{BART} & \multicolumn{7}{c}{GPT3} \\
% % encoding ↓ - task category → & question generation & answer generation & classifi-
% % cation & incorrect answer gen. & minimal
% % text mod. & verifi-
% % cation & avg & question generation & answer generation & classifi-
% % cation & incorrect answer gen. & minimal
% % text mod. & verifi-
% % cation & avg \\
% \cmidrule(r){2-8} \cmidrule(r){9-15} 
%  task category → & QG & AG & CF & IAG & MM & VF & avg & QG & AG & CF & IAG & MM & VF & avg \\
% \midrule
% No instruction & 26 & 6 & 0 & 21 & 33 & 7 & 13 & - & - & - & - & - & - & - \\
% \midrule
% prompt & 27 & 22 & 7 & 22 & 34 & \textbf{9} & 20  & 33 & 32 & 14 & 13 & \textbf{73} & 16 & 30 \\
% {\ \ \ +definition} & 35 & 24 & 50 & 25 & 36 & 7 & 30$\uparrow$ (+50) & 36 & 35 & 40 & 14 & 70 & 16 & 35 $\uparrow$ (+17)\\
% { \ \ \ +things to avoid} & 33 & 24 & 4 & 24 & \textbf{58} & \textbf{9} & 25$\uparrow$ (+25) & 28 & 33 & 11 & 16 & 68 & 14 & 28 $\downarrow$ (-7) \\
% %{\ \ \ +emphasis} & 38 & 23 & 16 & \textbf{26} & 49 & 3 & 26 & 29 & 28 & 18 & 16 & 72 & 16 & 30 \\
% {\ \ \ +pos. examp.} & 56 & 22 & 28 & 24 & 53 & 5 & 31$\uparrow$ (+55) & \textbf{43} & 49 & 29 & 21 & 70 & \textbf{36} & 41$\uparrow$ (+37) \\
% {\ \ \ +definition+pos. examp} & 55 & 23 & 50 & \textbf{26} & 54 & 7 & \textbf{36}$\uparrow$ (+80) & \textbf{43} & 50 & \textbf{45} & \textbf{23} & 70 & 32 & \textbf{44}$\uparrow$(+47) \\
% %{\ \ \ +pos, neg ex+ explan.} & 50 & 21 & 27 & 25 & 50 & 7 & 30 & 32 & 19 & 8 & 12 & 61 & 13 & 24 \\
% {pos. examples} & \textbf{57} & 6 & 9 & 25 & 49 & 7 & 26$\uparrow$ (+30) & 30 & 32 & 15 & 16 & 68 & 23 & 31$\uparrow$(+3) \\
% \midrule
% {Full Instruction} & 46 & 25 & 52 & 25 & 35 & 7 & 32$\uparrow$ (+60) & 33 & 18 & 8 & 12 & 60 & 11 & 24 $\downarrow$(-20) \\
% %{\ \ \ - examples } & 40 & 24 & 36 & 25 & 55 & 8 & 31 & 31 & 34 & 39 & 14 & 69 & 13 & 33 \\
% {\ \ \ - neg. examples} & 53 & \textbf{27} & \textbf{53} & 25 & 48 & 6 & 35$\uparrow$ (+75) & \textbf{43} & \textbf{54} & 44 & 21 & 70 & 32 & \textbf{44}$\uparrow$(+47) \\
% % \midrule 
% % Task-specific model & & & & &  & & & - & - & - & - & - & - & -  \\
% \bottomrule
% \end{tabular}
% }
%  \caption{
%     Cateogry wise results of BART and GPT3 for various input encodings, under random split (\S\ref{subsec:split}).
%     For both systems the addition of the instructions generally improves the model performance, as indicated
%         by the relative gains indicated in the `avg' columns (in percentage compared to ``prompt'' encoding.)
%         Category names: QG: Question Generation, AG: Answer Generation, CF: Classification, IAG: Incorrect Answer Generation, MM: Minimal Text Modification, VF: Verification.
%     }
%     \label{tab:random:splitfull}
% \end{table*}

\begin{comment}
\daniel{
Capacity of the proposed schema: 
We acknowledge that mapping crowdsoucing instructions to our schema is a lossy process. 
% , as plain text is not as representative as HTML templates. 
In the constructions we have tried to retain as much information as possible so that the resulting instructions are still faithful to the original task. 
% acknowledge that we change the template a bit; compared to what crowdworkers see; talk about verification
% In some cases, html information (e.g., certain organization of the information boxes) are lost while converting them into our schema. 
% We hope such issues will be addressed in future work. 
}
\end{commment}


% \cite{weller2020learning} -> ZEST dataset
% \cite{goldwasser2014learning} -> lesson interpretation problem ->  the learner is given a lesson describing the target concept directly and a few instances exemplifying it --> feedback is given to constrained interpretation program 
% cite{efrat2020turking} ->Turking Test, which examines a model’s ability to follow natural language instructions --> We begin with turking tasks (Section 3), where the model is tasked with creating valid dataset examples of popular NLP datasets (SNLI, SQuAD, and NewsQA), simulating a task commonly done by laypeople on crowdsourcing platforms 
% \cite{clark2020transformers} -> e the facts and rules are provided as natural language sentences, thus bypassing a formal representation.
% scale=0.70,trim=1.2cm 0.5cm 0cm 1.5cm



% Our experiments show the benefit of our comprehensive descriptions in better generalization capabilities. 
%In our experiments we show that models can benefit from detailed descriptions in these 
% Most of the works in this bucket explore ways to form natural language prompt for generative LMs, often for benchmarks like SuperGLUE~\cite{wang2019superglue}. 
% We see several limitations with this line of work:
% since there is no established benchmark for studying ``prompts'' (and more broadly, instructions), each work has a different setup for their study, which creates barriers for the reproducibility of the experiments.

% For example, \cite{scao2021many} uses prompts like the following for their question-answering subtask: \emph{ ``p. Based on the previous passage, q? <MASK>.''}. 
% \name{} can serve as a benchmark for the study of complex prompts formulated as natural language instructions. 
% Additionally, the diversity of the tasks in \name{} would allow the field to study generalization across subtasks by effective comprehension of the instruction --- one of the key motivations for this work. 

% \cite{shin2020autoprompt} ->  develop automatically-constructed prompts that elicit knowledge from pretrained MLMs for a variety of tasks 
% \cite{schick2020few} ->  introducing the concept of decoder prefixes and (ii) combining patterns through knowledge distillation  
% \cite{schick2020exploiting} -> We have shown that providing task descriptions to pretrained language models can be combined with standard supervised training. When the initial amount of training data is limited, PET gives large improvements over standard supervised training and strong semi-supervised approaches.
% \cite{schick2020s} -> t it is possible to achieve fewshot performance similar to GPT-3 on SuperGLUE with LMs that have three orders of magnitude fewer parameters 
% \cite{scao2021many} -> a task-specific promp / prompts provide a method for injecting taskspecific guidance, . By controlling for many sources of advantage, we find that prompting does indeed provide a benefit, and that this benefit can be quantified per task. Results show that prompting is often worth 100s of data
% \cite{liu2021gpt} -> ignore 
% \cite{li2021prefix} -> We have proposed prefix-tuning, a lightweight alternative to fine-tuning that prepends a trainable continuous prefix for NLG tasks. 
% \cite{ben2021pada} -> ignore 
% \cite{reynolds2021prompt} -> Using GPT-3 as a case study, we show that 0-shot prompts can significantly outperform few-shot prompts. We suggest that the function of few-shot examples in these cases is better described as locating an already learned task rather than meta-learning. 
% \cite{liu2021makes} ->  we propose to retrieve examples that are semantically-similar to a test sample to formulate its corresponding prompt.
% \cite{tam2021improving} -> focus on few shot learning without any unlabeled data and introduce ADAPET 
% \cite{zhao2021calibrate} -> We show that this type of few-shot learning can be unstable: the choice of prompt format, training examples, and even the order of the training examples can cause accuracy to vary from near chance to near state-of-the-art 


\begin{comment}
\begin{itemize}
    \item Learning from Task Descriptions \cite{goldwasser2014learning} \cite{weller2020learning} \cite{efrat2020turking} \cite{clark2020transformers} \cite{hase2021can} \cite{ye2021zero}
    \item Prompt Engineering \cite{scao2021many} \cite{shin2020autoprompt} \cite{liu2021gpt} \cite{li2021prefix} \cite{ben2021pada} \cite{reynolds2021prompt} \cite{liu2021makes}Pattern Expolited Training \cite{schick2020few} \cite{schick2020exploiting} \cite{schick2020s} \cite{tam2021improving} \cite{zhao2021calibrate}
    \item Semantic Parsing \cite{shao2020chartdialogs}\cite{lake2018generalization} 
    \cite{lin2018nl2bash}
     \cite{kulal2019spoc}\cite{walter2013learning}
    % \item Data Augumentation \cite{xie2019unsupervised} \cite{lee2021neural}
    % \item Question Decomposition \cite{shwartz2020unsupervised} \cite{khot2020text}
    % \item Controlled Text Generation \cite{dathathri2019plug}
\end{itemize}
\end{comment}




\begin{comment}
\begin{table}[]
    \centering
    \small
    \begin{tabular}{ccc}
        \toprule 
         Task  & \makecell{Cross-Task\\Generalization} & \makecell{Multi-Task\\Learning} \\
         \midrule 
         Training data & \makecell{$\{ (D_t, I_t) | t \in$\task{\color{blue} train} $\}$ \\ }  & \makecell{$\{ D_t | t \in$\task{\color{blue} train} $\}$ \\ } \\ 
         \midrule
         \makecell{Test-time\\Inference}  &  \makecell{$(I_t, x) \rightarrow y$ \\ for $(x, y) \in D_t$ \\ and $t \in $ \task{\color{red} test} }  & \makecell{$x \rightarrow y$ \\ for $(x, y) \in D_t$ \\ and $t \in $ \task{\color{blue} train}  }  \\ 
        \bottomrule
    \end{tabular}
    \caption{
        A comparison of \emph{cross-task generalization} and \emph{multi-task learning}. 
        In all above notations, $D_t$ refers to the collection of input-output instances for task $t$: $D_t=\{(x,y)|x \in X_t,y \in Y_t\}.$ 
        While multi-tasking is trained and evaluated on the same set of tasks \task{\color{blue} train}, the evaluation of cross-task generalization is done on  \task{\color{red} test} where \task{\color{red} test} $\cap$ \task{\color{blue} train}$ = \emptyset $. 
    }
    \label{tab:comparison}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[]
    \centering
    \small
    \begin{tabular}{ccc}
        \toprule 
        %  Task  & \makecell{Cross-Task\\Generalization} & \makecell{Conventional\\Setup} \\
        %  \midrule 
         \makecell{Training data} & \makecell{$\{ (I_t, X^{\text{train}}_t, Y^{\text{train}}_t) |  t \in \text{\task{\color{blue} seen}}  \}$ \\ }  \\ 
         \midrule 
         Evaluation & \makecell{ $\ell (M(x_, I_t), y_t)$ \\ where: \\ $(x, y) \in (X^{\text{test}}_t, Y^{\text{test}}_t)$,  $t \in$ \task{\color{red} unseen} } \\ 
        \bottomrule
    \end{tabular}
    \caption{
        % In all above notations, $D_t$ refers to the collection of input-output instances for task $t$: $D_t=\{(x,y)|x \in X_t,y \in Y_t\}.$ 
        In the conventional setup, training and evaluation is done on the same set of tasks, i.e., \task{\color{blue} seen} $=$ \task{\color{red} unseen} (and the task definitions $I_t$ do not play a major role for the known tasks).  
        In comparison, \emph{cross-task generalization} a model is expected to generalize to of {\color{blue} seen} tasks, where \task{\color{red} unseen} $\cap$ \task{\color{blue} seen}$ = \emptyset$. 
    }
    \label{tab:comparison}
\end{table}
\end{comment}



%Here we investigate whether one can build a model that has the \emph{generality} to solve various tasks by reading their \emph{instructions}, even if they are not seen apriori. 


% Unlike our elaborate instructions, these works were conducted on much short language prompts. 
% Additionally, since we represent the instructions in a structured format, we are able to ablate various elements of the instructions and quantify their contributions. 

% \daniel{
% There are two other contributions (beyond schema) that lead to cross-task generalization. 
% (1) Decomposing the crowdsourcing instructions into well-defined sub-tasks (aligned with crowdsourcing steps) leads to more informative and concise instructions. This is important since, as G2 shows, raw instructions are typically verbose. 
% (2) Large-scale supervision with instructions: 
% Having collected a dataset of 60+ tasks, we are able to train models on a subset of the tasks and generalize them to the remaining ones. We show that model generalization (to unseen tasks) increases with more observed tasks (Fig 5; green line) with instruction, in contrast to the conventional setup (no instructions) (Fig 5; blue line). 
% }


% Alas, the the dominant learning paradigm that uses task-specific labeled data to train models which rarely cannot generalize to new tasks. 

%We are also motivated by recent large pre-trained language models \cite{brown2020language} that have shown promising results when provided with a natural language prompt and a few task-specific  examples~\cite{schick2020s,scao2021many}.
%While these observations are encouraging, the currently studied  ``prompts'' are often too  simple, whereas many real NLP problems  cannot be effectively formulated as short ``prompts'' or a few positive examples. For example, instructions provided to crowdworkers are often much more detailed and nuanced than simple prompts.   %which limits our understanding of the extents of LMs capabilities. 
% in addressing them. 
%There are many real NLP problems that cannot be effectively formulated as short ``prompts'' or few positive examples. 
%An evidence of this in-the-wild is that the instructions 
% written for crowdsourcing datasets and 
%shown to crowdworkers are typically much more detailed and nuanced than simple prompts.  
% (e.g., finding essential keywords in a question, studied later in this work). 
% In fact, a recent study~\cite{efrat2020turking} show that these  models fail to learn three complex tasks (SNLI, SQuAD, NewsQA) given their crowdsourcing instructions.  %\cite{raffel2020exploring,brown2020language}



       % A long-standing challenge in AI is to  build a model equipped with the understanding of human-readable \emph{instructions} that define the tasks, which can generalize to new tasks.
    % \swaroop{\sout{A long-standing challenge in AI is to build a model that is equipped with the understanding of human-readable \emph{instructions} that define the tasks, and can generalize to new tasks.} 
    % \begin{comment}
    % The conventional NLP is often concerned with learning decision functions from labeled instances. 
    % While this paradigm has been successful in producing strong task-specific models, they fail to generalize across tasks (e.g., a question-answering system cannot solve  classification tasks).
    % We hypothesize that a model equipped with the understanding of  \emph{instructions} that define the tasks, can generalize to \emph{unseen} tasks. 
    % \end{comment}
    % (such as question-answering and classification). 
    % \swaroop{question answering and classification are pretty close, in fact classification can be also thought of as a question answering e.g. BoolQA. How about writing question answering and question generation.}
    % We hypothesize that for a model to generalize to novel tasks, it has to be equipped with the ability to comprehend task definition -- serving as a high-level representation of the task.
    % Backed by this modified setup, we advocate for studying
    % Enabled by this additional information, 
    % the question of whether one can build a single model that generalizes to novel tasks by an appropriate understanding of their instructions. 
    % \swaroop{I think we need to clarify 3 things. (i) Why what we are doing intuitively make sense? (ii) the phrase "assume labeled examples of each task are accompanied by their \emph{instructions}" gives an impression that creating instruction is an overhead and requires a lot of effort. Then people will start thinking whether this effort is wort it? (iii) when we say labelled examples, we ignore GPT3 setup. Also the word "labelled examples" will upset some reviewers who are tired of supervised learning setup. My suggestion: "Humans learn from a diverse set of tasks which is a challenge for machines (UnifiedQA is limited to a narrow range of tasks). Humans implicitly have background knowledge about tasks that help them relate different tasks and generalize. We are interested in studying "Can we provide instructions along with data samples and help model generalize better?" Additionally, Instruction paradigm can help a lay person to get benefited by NLP as they do not need to curate a lot of samples to enable a model do the desired task. So we intend to study "Can we enable NLP models to appropriately respond to instructional prompts and consequently generalize to new tasks?""}
% Can we enable NLP models to appropriately respond to instructional prompts and consequently generalize to new tasks? 
% \hanna{I am trying to write this sentence more precisely, see if you agree?}
% \daniel{reads well to me}s
% To study this question, we leverage the existing NLP datasets and their corresponding crowdsourcing instructions to create 

% Using large pre-trained models show significant advances in many NLP datasets and benchmarks....
% Furthermore, recent work has built unified models  using multi-task training over several datasets within a known NLP task ( e.g., QA~\cite{unifiedQA}, xxx~\cite{xxx}). However, many tasks 


\begin{comment}
\begin{table}[t]
    \small 
    \centering
    % \resizebox{\linewidth}{!}{
\begin{tabular}{lcc|cc}
\toprule 
& \multicolumn{2}{c}{BART} & \multicolumn{2}{c}{GPT3} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} 
& \makecell{avg} & \makecell{gains } & \makecell{avg} & \makecell{gains } \\
\midrule
No instruction & 13 & - & - & - \\
\midrule
prompt & 20 & 0.0 & 30.0 & 0.0 \\
{\ \ \ +definition} & 30 & 50.0$\uparrow$ & 35.0 & 16.7$\uparrow$ \\
{ \ \ \ +things to avoid} & 25 & 25.0$\uparrow$ & 28.0 & -6.7$\downarrow$ \\
{\ \ \ +emphasis} & 26 & 30.0$\uparrow$ & 30.0 & 0.0 \\
{\ \ \ +pos. examp.} & 31 & 55.0$\uparrow$ & 41.0 & 36.7$\uparrow$ \\
% prompt+positive/negative examples + explanations & 30 & 50.0 & 24.0 & -20.0 \\
% {\ \ \ +definition+pos. examp} & \bf{36} & 80.0$\uparrow$ & \bf{44.0} & 46.7$\uparrow$ \\
{pos. examples} & 26 & 30.0$\uparrow$ & 31.0 & 3.3$\uparrow$ \\ 
\bottomrule
{Full Instruction} & 32 & 60.0$\uparrow$ & 24.0 & -20$\downarrow$ \\
{\ \ \ - examples } & 31 & 55.0$\uparrow$ & 33.0 & 10.0$\uparrow$ \\
{\ \ \ - neg. examples} & 35 & 75.0$\uparrow$ & \bf{44.0} & 46.7$\uparrow$ \\
\bottomrule
\end{tabular}    
% }
    \caption{
        Evaluating BART and GPT3 with \setup{1} split (Table~\ref{tab:supervision:types}). \hanna{in caption say the gains are w.r.t prompt}\daniel{the last sentence says it.}
        % Empirical results NATURAL-INSTRUCTIONS.
        % The first row is a task-specific model with no instances.
        % This model serves as our upper-bound, which is why it is grayed out. 
        For each of the two systems (BART and GPT3), we see that the addition of the instructions helps propel the model performance, as indicated
        by the relative gains \swaroop{in percentage} compared to
        ``prompt'' encoding.
    }
    \label{tab:random:split}
\end{table}
\end{comment}

